Reinforcement Learning Approach to Active Learning for Image Classification

Machine Learning requires large amounts of labeled data to fit a model. Many datasets are already publicly available, nevertheless forcing application possibilities of machine learning to the domains of those public datasets. The ever-growing penetration of machine learning algorithms in new application areas requires solutions for the need for data in those new domains. This thesis works on active learning as one possible solution to reduce the amount of data that needs to be processed by hand, by processing only those datapoints that specifically benefit the training of a strong model for the task. A newly proposed framework for framing the active learning workflow as a reinforcement learning problem is adapted for image classification and a series of three experiments is conducted. Each experiment is evaluated and potential issues with the approach are outlined. Each following experiment then proposes improvements to the framework and evaluates their impact. After the last experiment, a final conclusion is drawn, unfortunately rejecting this work's hypothesis and outlining that the proposed framework at the moment is not capable of improving active learning for image classification with a trained reinforcement learning agent.

==> chapters/methUncertaintySampling.tex <==
\subsection{Uncertainty Sampling} \label{sec:uncertaintySampling}
The most common sampling strategy is to pick the instance from $U$ for which the model is most ``unsure''. This is straightforward for probabilistic models as they provide their certainty in the output. Different metrics can be employed to evaluate the uncertainty (\cite{alSurvey}  pp. 12-15):\\
(i) The least confident value among all of the highest class probabilities
\begin{align*}
    x^\star = \underset{x \in U}{argmax} \hspace{2mm} 1 - P_\Theta(\hat y| x) \\
    with \hspace{4mm} \hat y = \underset{y}{argmax} \hspace{2mm} P_\Theta(y| x)
\end{align*}
(ii) The difference between the the highest and second highest class probability, also known as ``Best vs Second Best'' (BvsSB)
\begin{equation*}
    x^\star = 1 - \underset{x \in U}{argmin} \hspace{2mm} P_\Theta(\hat y_1| x) - P_\Theta(\hat y_2| x)
\end{equation*}
(iii) The Shannon entropy over the class probabilities
\begin{equation*}
    x^\star = \underset{x \in U}{argmax} \hspace{1.5mm} - \sum\limits_i P_\Theta(\hat y_i| x) log P_\Theta(\hat y_i| x)
\end{equation*}
A visual comparison of the sampling strategies can be found in below. The graphs picture a 3 class scenario where the position within the triangle represents the probability for each of the three classes, given an instance and the color represents the most informative areas.
\begin{figure}[h]
    \begin{center}
        \includegraphics[width=\textwidth]{figs/alStrategyHeatmap}
    \end{center}
    \caption*{\hspace{-5mm} (i) least confident \hspace{17mm} (ii) BvsSB \hspace{25mm} (iii) Entropy}
    \caption{Most informative areas in a 3 class problem according to the sampling strategies (\cite{alSurvey} Fig. 5)}
\end{figure}
Each strategy shares the property that the most informative samples can be found in the middle of the triangle, where the probability for each class is leveled at $\frac{1}{3}$, and the least informative samples are at the corners, where one class a probability of 1 and the rest has 0. However, they differ in the rest of the probability space. Strategy (i) and (iii) both are very centralised, favoring those instances that produce a low overall confidence in the prediction. Strategy (iii) only focuses on the two highest probabilities, favoring a high uncertainty between those two. By doing this, the BvsSB strategy solves a common problem of (i) and (iii). When dealing with problems with a large number of labels, the probability distribution $P_\Theta(\hat y| x)$ tends to flatten out towards all the unlikely labels. This lowers the confidence of more likely labels compared to the mass of unlikely labels, as well as causing a high entropy for every sample $x \in U$. This hinders the performance of the \textit{least confident} (i) and entropy (iii) strategy.

